Graph2Seq: Scalable Learning Dynamics for Graphs

Neural networks have been shown to be an effective tool for learning algorithms over graph-structured data. However, graph representation techniques---that convert graphs to real-valued vectors for use with neural networks---are still in their infancy. Recent works have proposed several approaches (e.g., graph convolutional networks), but these methods have difficulty scaling and generalizing to graphs with different sizes and shapes. We present Graph2Seq, a new technique that represents vertices of graphs as infinite time-series. By not limiting the representation to a fixed dimension, Graph2Seq scales naturally to graphs of arbitrary sizes and shapes. Graph2Seq is also reversible, allowing full recovery of the graph structure from the sequences. By analyzing a formal computational model for graph representation, we show that an unbounded sequence is necessary for scalability. Our experimental results with Graph2Seq show strong generalization and new state-of-the-art performance on a variety of graph combinatorial optimization problems.

==> arxiv 3/architecture.tex <==
\section{Neural Network Design} \label{sec: Neural Network Design}
% We demonstrate \algo~on the following combinatorial optimization problems: minimum vertex cover (MVC), maximum cut (MC) and maximum independent set (MIS).
% These are well-known to be NP-hard, and also have varying hardness of approximation.
% For e.g. minimum vertex cover can be approximated to within a factor of 2~\citep{papadimitriou1998combinatorial},\footnote{However it is known to be hard to approximate beyond a factor of 1.36~\citep{dinur2002importance}.} while the maximum independent set problem cannot be approximated to within $O(n^{1-\epsilon})$ for any constant $\epsilon > 0$ on a graph of size $n$ unless $P=NP$~\citep{williamson2011design}.
% The problems also admit input graph instances of arbitrary size, allowing us to test and demonstrate scalability of \algo.
% In the following sections we discuss the learning algorithm, and the neural network architecture.

We consider a reinforcement learning (RL) formulation for combinatorial optimization problems on graphs. RL is well-suited to such problems since the true  `labels' (i.e., the optimal solution) may be unavailable or hard to compute. 
Additionally, the objective functions in these problems can be used as natural reward signals.
An RL approach has been explored in recent works~\citet{vinyals2015pointer, bello2016neural, dai2017learning} under different representation techniques.  
Our learning framework uses the \algo~representation.
Fig.~\ref{fig: neural arch} shows our neural network architecture. 
We feed the trajectories output by \algo for all the vertices into a recurrent neural network (specifically RNN-GRU), whose outputs are then aggregated by a feedforward network to select a vertex. 
Henceforth we call this the \gtos neural network architecture. 
The key feature of this design is that the length of the sequential representation is {\em not} fixed; we vary it depending on the input instance. 
We show that our model is able to learn rules---for both generating the sequence and processing it with the RNN---that generalize to operate on long sequences.
In turn, this translates to algorithmic solutions that scale to large graph sizes.

% \noindent {\em Adversarial training}. Another important reason for \algo's generalization
% capability is our careful adversarial choice of the training set.
% The combinatorial problems naturally allow us to present `hard examples'   for training.
% By choosing an adversarial set of example graphs, we demonstrate the corresponding model  generalizes
% much better both in terms of graph structure and graph size, compared to GCNN methods in the literature.
%The learning algorithm and neural network architecture are elaborated in the following.

%\begin{figure}[t]
%  \centerline{\includegraphics[height=40mm]{figures/neural_arch}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%     \label{fig: neural arch}}
%    \caption{Neural network architecture.}
%%    \label{fig: Graph2Seq}
%\end{figure}

\noindent {\bf Reinforcement learning model.} We consider a RL formulation in which vertices are chosen {\em one at a time}. 
Each time the RL agent chooses a vertex, it receives a reward.
The goal of training is to learn a policy such that cumulative reward is maximized.
We use  $Q$-learning to train the network.
\begin{wrapfigure}{l}{0.55\textwidth} 
%\begin{figure}[t] 
\vspace{0pt}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{./figures/neural_arch.png}
    \caption{\small The \gtos neural network architecture. The GRU units process the representation output by \algo, operating independently on each vertex's time-series.}
    \label{fig: neural arch}
  \end{center}
  \vspace{-12pt}
% \end{figure} 
\end{wrapfigure} 
For input graph instance $G(V,E)$, a subset $S\subseteq V$ and $a\in V\backslash S$, this involves using a neural network to approximate a $Q$-{\em function} $Q(G,S,a)$. Here $S$ represents the set of vertices already picked.
% In the following we describe the neural network to compute $Q(G,S,a)$.
The neural network comprises of three modules:
% \begin{enumerate} [noitemsep, topsep=0pt]
% \item
(1) {\em Graph2Seq}, that takes as input the graph $G$ and set $S$ of vertices chosen so far. It generates a sequence of vectors as output for each vertex.
% \item 
(2) {\em Seq2Vec} reads the sequences output of \algo and summarizes it into one vector per vertex.
% \item
(3) $Q$-{\em Network} takes the vector summary of each vertex $a \in V$ and outputs the estimated $Q(G,S,a)$ value. 
% \end{enumerate}
The overall architecture is illustrated in Fig.~\ref{fig: neural arch}.
To make the network practical, we truncate the sequence outputs of \algom~to a length of $T$.
However the value of $T$ is not fixed, and is varied both during training and testing according to the size and complexity of the graph instances encountered; see \S~\ref{sec: evals} for details.
We describe each module below.

{\bf Graph2Seq.}
% We consider a $d$-dimensional state-space in which the dynamics of each vertex evolves.
Let $\mathbf{x}_v(t)$ denote the state of vertex $v$ and $c_v(t)$ denote the binary variable that is one if $v \in S$ and zero otherwise, at time-step $t$ in the \algo evolution.
Then, the trajectory of each vertex $v\in V$ evolves as
% \begin{align}
$ \mathbf{x}_v(t+1) = \mathrm{relu} (
 \mathbf{W}_{G,1} \sum_{u\in\Gamma(v)}\mathbf{x}_u(t) + \mathbf{w}_{G,2} c_v(t) + \mathbf{w}_{G,3} ),$ 
% \end{align}
for $t=0,1,\ldots, T-1$. 
$\mathbf{W}_{G,1}\in\mathbb{R}^{d\times d}, \mathbf{w}_{G,2}\in\mathbb{R}^d, \mathbf{w}_{G,3}\in\mathbb{R}^d$ are trainable parameters, and $\mathbf{x}_v(0)$ is initialized to all-zeros for each $v\in V$.

{\bf Seq2Vec and $Q$-Network.}
The sequences $\{ (\mathbf{x}_v(t))^T_{t=1}: v \in V\} $ are processed by GRU units~\citep{chung2014empirical} at the vertices. 
% that read $\mathbf{x}_v(\cdot)$ vectors at each time index for all $v\in V$.
At time-step $t$, the recurrent unit at vertex $v$ computes as input a function that depends on (i) $\mathbf{x}_v(t)$, the embedding for node $v$, (ii) $\sum_{u\in\Gamma(v)}\mathbf{x}_u(t)$, the neighboring node embeddings and (iii) $\sum_{u\in V}\mathbf{x}_u(t)$, a summary of embeddings of all nodes. 
This input is combined with the GRU's cell state $\mathbf{y}_v(t-1)$ to produce an updated cell state $\mathbf{y}_v(t)$.
The cell state at the final time-step $\mathbf{y}_v(T)$ is the desired vector summary of the \algo~sequence, and is fed as input to the $Q$-network.
We refer to Appendix~\ref{sec: net arch appendix} for equations on Seq2Vec. 
%let $\mathbf{y}_v(t) \in \mathbb{R}^d$ be the $d$-dimensional cell state, $\mathbf{i}_v(t)\in\mathbb{R}^d$ be the cell input and $\mathbf{f}_v(t) \in (0,1)^d$  be the forgetting gate, for each vertex $v\in V$.
%Each time-step a fresh input $\mathbf{i}_v(t)$ is computed based on the current states $\mathbf{x}_u(t)$ of $v$'s neighbors in $G$.
%The cell state is updated as a convex combination of the freshly computed inputs $\mathbf{i}_v(t)$ and the previous cell state $\mathbf{y}_v(t-1)$, where the weighting is done according to a forgetting value $\mathbf{f}_v(t)$ that is also computed based on the current vertex states.
%The precise update equations for the input vector, forgetting value and cell state have been presented in Appendix C.
%   chosen as follows:
%\begin{align}
%\mathbf{i}_v(t+1) &= \mathrm{relu} ( \mathbf{W}_4 \sum_{u\in\Gamma(v)} \mathbf{x}_v(t) + \mathbf{w}_5 c_v(t) + \mathbf{b}_6 ) \notag \\
%\mathbf{f}_v(t+1) &= \mathrm{sigmoid} ( \mathbf{W}_7 \sum_{u\in V} \mathbf{x}_u(t) + \mathbf{b}_8 ) \notag \\
%\mathbf{y}_v(t+1) &= \mathbf{f}_v(t+1) \odot \mathbf{i}_v(t+1) + (\mathbf{1}-\mathbf{f}_v(t+1)) \odot \mathbf{y}_v(t),
%\end{align}
%where $\mathbf{W}_4, \mathbf{W}_7 \in \mathbb{R}^{d\times d}$ and $\mathbf{w}_5, \mathbf{b}_6, \mathbf{b}_8 \in \mathbb{R}^d$ are trainable parameters,  $t=0,1,\ldots,T-1$, and $\mathbf{1}$ denotes the $d$-dimensional all-ones vector, and $\odot$ is element-wise multiplication. $\mathbf{y}_v(0)$ is initialized to all-zeros for every $v\in V$.
The $Q$-values are estimated as 
\begin{align}
\tilde{Q}(G,S,v) = &\mathbf{w}_{Q,1}^T \mathrm{relu} ( \mathbf{W}_{Q,2} \sum_{u\in V} \mathbf{y}_u(T) ) 
+ \mathbf{w}_{Q,3}^T \mathrm{relu} \left( \mathbf{W}_{Q,4} \mathbf{y}_v(T) \right), \label{eq: Q func est}
\end{align}
with $\mathbf{W}_{Q,1}, \mathbf{W}_{Q,3} \in \mathbb{R}^{d\times d}$ and $\mathbf{w}_{Q,2}, \mathbf{w}_{Q,4} \in \mathbb{R}^d$ being learnable parameters.
All transformation functions in the network leading up to~\eqref{eq: Q func est} are differentiable.
This makes the whole network differentiable, allowing us to train it end to end. 

{\bf Remark.}
In Fig.~\ref{fig: neural arch} the \algo RNN and the GRU RNN can also be thought of as two layers of a two-layer GRU. 
We have deliberately separated the two RNNs to highlight the fact that the sequence produced by \algo (blue in Fig,~\ref{fig: neural arch}) is the embedding of the graph, which is then read using a GRU layer (red in Fig.~\ref{fig: neural arch}).  
Our architecture is not unique, and other designs for generating and/or reading the sequence are possible.
% Combining the LSTM units with the graph convolution layers may indeed work well as long as the final output is based on the entire sequence of convolution operations.



% Next we describe the general training and testing techniques used in the evaluations.


%compute the (stochastic) gradients of the loss function in Equation~\eqref{eq: emp loss} for learning.
% Having a well-defined scalar objective function allows us to choose the `best' solution among all solutions generated by varying the sequence length hyper-parameter.
% We also observe in our evaluations that the quality of solutions generated is not monotonically improving as we increase $T$.
% This phenomenon is discussed more in Section~\ref{sec: ablation analysis}.

%We test generalization in graph structure and size.
%Using the {\em same} trained parameters, we test \algo~on the following broad graph classes: Erdos-Renyi graphs, bipartite graphs, regular graphs and structured examples, while varying the graph sizes between 25--3200.

% - time complexity analysis?
% - notation: layer vs round vs iteration, dynamics vs evolutions vs trajectory

















==> arxiv 3/background.tex <==
\section{Background: Graph Convolutional Neural Networks} \label{sec: background}

% A key towards developing a good learning algorithm for problems with input data structured as (or over) a graph, is to first have an efficient representation for the input graph.
An ideal graph representation is one that captures all innate structures of the graph relevant to the task at hand, and moreover can also be learned via gradient descent methods.  %\footnote{This latter requirement could be relaxed. For e.g., it may be possible to develop a static (task independent) representation for graphs such as using its Laplacian matrix. We do not consider such a representation, but recognize it as an important future direction.}
However, this is challenging since the relevant structures could range anywhere from local attributes (example: node degrees) to long-range dependencies spanning across a large portion of the graph (example: does there exist a path between two vertices)~\citep{kuhn2016local}.
Such broad scale variation is also a well-known issue in computer vision (image classification, segmentation etc.), wherein convolutional neural network (CNN) designs have been used quite successfully~\citep{krizhevsky2012imagenet}.
Perhaps motivated by this success, recent research has focused on generalizing the traditional CNN architecture to develop designs for graph convolutional neural networks (GCNN)~\citep{bruna2013spectral, niepert2016learning}.
By likening the relationship between adjacent pixels of an image to that of adjacent nodes in a graph, the GCNN seeks to emulate CNNs by defining localized `filters' with shared parameters.

Current GCNN filter designs can be classified into one of two categories: {\em spatial}~\citep{kipf2016semi, dai2017learning, nowak2017note}, and {\em spectral}~\citep{defferrard2016convolutional}.
For an integral hyper-parameter $K\geq 0$, filters in either category process information from a $K$-local neighborhood surrounding a node to compute the output. Here we consider localized spectral filters such as proposed in~\citet{defferrard2016convolutional}.
The difference between the spatial and spectral versions arises in the precise way in which the aggregated local information is combined.


\noindent {\em Spatial GCNN}. For input feature vector $\mathbf{x}_v$ at each node $v\in V$ of a graph $G$, a spatial filtering operation is the following:
\begin{align}
\mathbf{y}_v = \sigma\left( \sum_{k=0}^{K-1} \mathbf{W}_k \left(\sum_{u\in V} (\tilde{\mathbf{A}}^k)_{v,u} \mathbf{x}_u\right) + \mathbf{b}_0 \right) \quad \forall v \in V,  \label{eq: spatial update}
\end{align}
where $\mathbf{y}_v$ is the filter output, ${\bf W}_k, k=1,\ldots,K$ and ${\bf b}_0$ are learnable parameters, and $\sigma$ is a non-linear activation function that is applied element-wise.
$\tilde{\mathbf{A}} = \mathbf{D}^{-1/2}\mathbf{A}\mathbf{D}^{-1/2}$ is the normalized adjacency matrix, and $\mathbf{D}$ is the diagonal matrix of vertex degrees.
Use of un-normalized adjacency matrix is also common. 
The $k$-power of the adjacency matrix selects nodes a distance of at most $k$ hops from $v$.
ReLU is a common choice for $\sigma$.
We highlight two aspects of spatial GCNNs: (i) the feature vectors are aggregated from neighboring nodes directly specified through the graph topology, and (ii) the aggregated features are summarized via an addition operation.


\noindent {\em Spectral GCNN}. Spectral GCNNs  use the notion of graph Fourier transforms to define convolution operation as the inverse transform of multiplicative filtering in the Fourier domain.
Since this is a non-local operation potentially involving data across the entire graph, and moreover it is computationally expensive to compute the transforms, recent work has focused on approximations to produce a local spectral filter of the form
\begin{align}
\mathbf{y}_v = \sigma \left( \sum_{k=0}^{K-1} \mathbf{W}'_k \left( \sum_{u \in V}  (\tilde{{\bf L}}^k)_{v,u} \mathbf{x}_u \right) + \mathbf{b}'_0 \right) \quad \forall v \in V,  \label{eq: spectral update}
\end{align}
where $\tilde{{\bf L}} = \mathbf{I} - \tilde{\mathbf{A}}$ is the normalized Laplacian of the graph, $(\tilde{{\bf L}}^k)_{v,u}$ denotes the entry at the row corresponding to vertex $v$ and column corresponding to vertex $u$ in $\tilde{{\bf L}}^k$, and ${\bf W}'_k, {\bf b}'_0$ are parameters~\citep{defferrard2016convolutional, kipf2016semi}.
As in the spatial case, definitions using unnormalized version of Laplacian matrix are also used. 
$\sigma$ is typically the identity function here.
The function in~\eqref{eq: spectral update} is a local operation because the $k$-th power of the Laplacian, at any row $v$, has a support no larger than the $k$-hop neighborhood of $v$.
Thus, while the aggregation is still localized, the feature vectors are now weighted by the entries of the Laplacian before summation.



\noindent {\em Spectral and Spatial GCNN are equivalent}. The distinction between spatial and spectral convolution designs is typically made owing to their seemingly different definitions.
However we  show that both designs are mathematically equivalent in terms of their representation capabilities.
\begin{prop}
Consider spatial and spectral filters in~\eqref{eq: spatial update} and~\eqref{eq: spectral update}, using 
%normalized adjacency and Laplacian matrices respectively.
the same nonlinear activation function $\sigma$ and $K$.
Then, for graph $G(V,E)$, for any choice of parameters ${\bf W}_k$ and ${\bf b}_0$ for $k=1,\ldots,K$ there exists parameters $\mathbf{W}'_k$ and $\mathbf{b}'_0$ such that the filters represent the same transformation function, and vice-versa.
\end{prop}
%(Proof in Appendix)
\begin{proof}
Consider a vertex set $V = \{1,2,\ldots,n\}$ and $d$-dimensional vertex states $\mathbf{x}_i$ and $\mathbf{y}_i$ at vertex $i\in V$.
Let $\mathbf{X} = [\mathbf{x}_1,\ldots,\mathbf{x}_n]$ and $\mathbf{Y} = [\mathbf{y}_1,\ldots,\mathbf{y}_n]$ be the matrices obtained by concatenating the state vectors of all vertices.
Then the spatial transformation function of~\eqref{eq: spatial update} can be written as
\begin{align}
\mathbf{Y} = \sigma\left( \sum_{k=0}^{K-1} \mathbf{W}_k \mathbf{X} \tilde{\mathbf{A}}^k + \mathbf{b}_0 \mathbf{1}^T \right), \label{eq: spatial mat version}
\end{align}
while the spectral transformation function of~\eqref{eq: spectral update} can be written as
\begin{align}
\mathbf{Y} &= \sigma \left( \sum_{k=0}^{K-1} \mathbf{W}'_k \mathbf{X} \tilde{\mathbf{L}}^k + \mathbf{b}'_0 \mathbf{1}^T \right) \\
&=  \sigma \left( \sum_{k=0}^{K-1} \mathbf{W}'_k \mathbf{X} (\mathbf{I} - \tilde{\mathbf{A}})^k + \mathbf{b}'_0 \mathbf{1}^T \right) \label{eq: lap defn} \\
&=  \sigma \left( \sum_{k=0}^{K-1} \mathbf{W}'_k \mathbf{X} \sum_{i=0}^k \binom{k}{i}(-1)^{k-i} \tilde{\mathbf{A}}^i + \mathbf{b}'_0 \mathbf{1}^T \right) \label{eq: mat binom thm} \\
&= \sigma \left( \sum_{k=0}^{K-1} \left( \sum_{i=k}^{K-1} \mathbf{W}'_i \binom{i}{k}(-1)^{i-k} \right) \mathbf{X} \tilde{\mathbf{A}}^k +  \mathbf{b}'_0 \mathbf{1}^T  \right). \label{eq: spectral mat version}
\end{align}
The~\eqref{eq: lap defn} follows by the definition of the normalized Laplacian matrix, and~\eqref{eq: mat binom thm} derives from binomial expansion.
To make the transformation in~\eqref{eq: spatial mat version} and~\eqref{eq: spectral mat version} equal, we can set
\begin{align}
\sum_{i=k}^{K-1} \mathbf{W}'_i \binom{i}{k}(-1)^{i-k} = \mathbf{W}_k, \quad \forall ~0\leq k\leq K-1,
\end{align}
and check if there are any feasible solutions for the primed quantities.
Clearly there are, with one possible solution being  $\mathbf{b}'_0 = \mathbf{b}_0$ and
\begin{align}
\mathbf{W}'_{K-1} &= \mathbf{W}_{K-1} \\
\mathbf{W}'_{k} &= \mathbf{W}_k - \sum_{i=k+1}^{K-1} \mathbf{W}'_i \binom{i}{k} (-1)^{i-k},  
\end{align}
$\forall ~0 \leq k \leq K-2.$
Thus for any choice of values for $\mathbf{W}_k, \mathbf{b}_0$ for $k=0,\ldots, K-1$ there exists $\mathbf{W}'_k, \mathbf{b}'_0$ for $k=0,\ldots,K-1$ such that the spatial and spectral transformation functions are equivalent.
The other direction (when $\mathbf{W}'_k$ and $\mathbf{b}_0$ are fixed), is similar and straightforward.
\end{proof}

Depending on the application, the convolutional layers may be supplemented with pooling and coarsening layers that summarize outputs of nearby convolutional filters to form a progressively more compact spatial representation of the graph.
This is useful in classification tasks where the desired output is one out of a few possible classes~\citep{bruna2013spectral}.
For applications requiring decisions at a per-node level (e.g. community detection), a popular strategy is to have multiple repeated convolutional layers that compute vector representations for each node, which are then processed to make a decision~\citep{dai2017learning, bruna2017community, nowak2017note}.
The conventional wisdom here is to have as many layers as the diameter of the graph, since filters at each layer aggregate information only from nearby nodes.
Such a strategy is sometimes compared to the message passing algorithm~\citep{gilmer2017neural}, though the formal connections are not clear as noted in~\citet{nowak2017note}.
Finally the GCNNs described so far are all end-to-end differentiable and can be trained using mainstream techniques for supervised, semi-supervised or reinforcement learning applications.

Other lines of work use ideas inspired from word embeddings for graph representation~\citep{grover2016node2vec, perozzi2014deepwalk}. Post-GCNN representation,  LSTM-RNNs have been used to analyze time-series data structured over a graph.
\citet{seo2016structured} propose a model which combines GCNN and RNN to predict moving MNIST data.
~\citet{liang2016semantic} design a graph LSTM for semantic object parsing in images.

%While the GCNN designs  proposed so far are promising as general-purpose frameworks for computation over graphs, there are critical shortcomings.
%As with other areas in deep learning, GCNN research tends to be validated on practical problems involving real-world datasets.
%In such instances, it is often the case that the sample `input size'  encountered during training and testing are similar in scale.
%However, in applications such as combinatorial optimization over graphs, ideally we seek the neural network to learn a heuristic that can be generalized to graphs of arbitrary size.
%Indeed the plethora of approximation heuristics (and optimal algorithms, wherever possible) proposed for graph optimization problems are predominantly of this form (e.g.~\citet{shimizu2016fast, christofides1976worst, goemans1995improved}).
%The performance of such heuristics may vary across input instances of different topologies and size;
%however, typically at least within a reasonable class of graph topologies these heuristics tend to perform consistently well regardless of the graph size (e.g. belief-propagation on trees).
%
%Unfortunately the GCNN designs proposed so far fall short in this regard.
%A vast majority of the prior work use as training and test samples graphs of similar size.
%The absence of generalization in scale is not for lack of trying -- we argue that existing GCNN architecture are fundamentally limited in their generalizations capability with respect to graph size.
%A key reason for this is that prior architectures represent the input graphs using a GCNN of a fixed depth.
%This depth is typically chosen to be of the order of the graph diameter, with the reasoning that information from every node in the graph, located howsoever apart, can all be aggregated (through the convolutional layers) for making the decision at the output layer.
%However as the input graph scales in size, its diameter may exceed the neural network depth leading to a situation where the span of the graph from which each neuron receives information is limited.
%While for some applications such local representations of nodes may suffice, in general it could be restrictive.


==> arxiv 3/conclusion.tex <==
\section{Conclusion}
%- are there other architectures that are fundamentally different from local methods?
%- can this approach be applied to other problems involving graphs (such as classification)?
%- how to solve changing number of layers each time?


%- open question: how to systematically design the training examples for general problems?

We proposed \algo~ that represents vertices of graphs as infinite time-series of vectors. The representation melds naturally with modern RNN architectures that take time-series as inputs. We applied this combination to three canonical combinatorial optimization problems on graphs, ranging across the complexity-theoretic hardness spectrum. Our empirical results best state-of-the-art approximation algorithms for these problems on a variety of graph sizes and types. In particular, \algo exhibits significantly better scalability and generalization than existing GCNN representations in the literature.  An open direction involves a more systematic study of the capabilities of \algo across the panoply of graph combinatorial optimization problems, as well as its performance in concrete (and myriad) downstream applications. 
Another open direction involves interpreting the policies learned by \algo to solve specific combinatorial optimization problems (e.g., as in LIME \citep{ribeiro2016should}). 
% Traditional approaches to bound the worst-case approximation ratio for graph algorithms appears impossible in the case of neural network methods---
% Exploring modern interpretability techniques in machine learning (e.g., LIME \cite{ribeiro2016should}) is of particular interest. 
A detailed analysis of the \algo dynamical system to study the effects of sequence length on the representation is also an important direction. 


==> arxiv 3/evaluation1.tex <==
\section{Evaluations} \label{sec: evals}

% \begin{wrapfigure}{r}{0.55\textwidth} 
\begin{figure}[t]
  \centerline{\subfigure[]{\includegraphics[height=32mm]{figures/scalability/scalability.pdf}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: scalability}}
%     \subfigure[]{\includegraphics[height=25mm]{figures/scalability/bipartite}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%    \label{fig: scalability_bipartite}}
%     \subfigure[]{\includegraphics[height=20mm]{figures/table}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%    \label{fig: large table}}    
    \subfigure[]{
    	{\scriptsize
    	\begin{tabular}[b]{ccc}
		\hline
		Heuristic & $10k$ nodes & $25k$ nodes \\
		\hline
		Graph2Seq (ER) & 6444 & 16174 \\
		Structure2Vec (ER) & 6557 & 16439 \\
		\hline 
		Graph2Seq (bipartite) & 5026 & 12603 \\
		Structure2Vec (bipartite) & 5828 & 14409 \\
		\hline
		\smallskip 
		\smallskip
		\smallskip
		\smallskip
    	\end{tabular}
	}
    \label{fig: large table}	
    }
}
    \caption{\small Scalability of \gtos~and GCNN in (a) Erdos-Renyi graphs (left), random bipartite graphs (right), and (b) on much larger graphs. The neural networks have been trained over the same graph types as the test graphs. Error bars show one standard deviation.}
    \label{fig: scalabilityfull}
    \vspace{-10pt}
\end{figure}
% \end{wrapfigure}


In this section we present our evaluation results for \algo.
We address the following central questions: 
(1) How well does \gtos~scale?
(2) How well does \gtos~generalize to new graph types? 
(3) Can we apply \gtos~to a variety of problems? 
(4) Does adversarial training improve scalability and generalization? 
To answer these questions, we experiment with \gtos on three classical graph optimization problems: minimum vertex cover (MVC), max cut (MC) and maximum independent set (MIS). 
These are a set of problems well known to be NP-hard, and also greatly differ in their structure~\citep{williamson2011design}.
We explain the problems below. 

\noindent {\bf Minimum vertex cover.}
The MVC of a graph $G(V,E)$ is the smallest cardinality set $S\subseteq V$ such that for every edge $(u,v) \in E$ at least one of $u$ or $v$ is in $S$.
Approximation algorithms to within a factor 2 are known for MVC; however it cannot be approximated better than 1.3606 unless P$=$NP. \\
\noindent {\bf Max cut.}
In the MC problem, for an input graph instance $G(V,E)$ we seek a cut $(S, S^c)$ where $S\subseteq V$ such that the number of edges crossing the cut is maximized. 
This problem can be approximated within a factor 1.1383 of optimal, but not within 1.0684 unless P$=$NP.  \\
\noindent {\bf Maximum independent set.}
For a graph $G(V,E)$ the MIS denotes a set $S\subseteq V$ of maximum cardinality such that for any $u, v\in S$, $(u,v) \notin E$. 
The maximum independent set is complementary to the minimum vertex cover---if $S$ is a MIC of $G$, then $V \backslash S$ is the MVC. 
However, from an approximation standpoint, MIS is hard to approximate within $n^{1-\epsilon}$ for any $\epsilon > 0$, despite constant factor approximation algorithms known for MVC.

\noindent {\bf Heuristics compared.}
In each problem, we compare \gtos~against:
(1) Structure2Vec~\citep{dai2017learning}, 
(2) GraphSAGE~\citep{hamilton2017inductive} using (a) GCN, (b) mean and (c) pool aggregators, 
(3) WL kernel NN~\citep{lei2017deriving}, 
(4) WL kernel embedding, in which the feature map corresponding to WL subtree kernel of the subgraph in a 5-hop neighborhood around each vertex is used as its vertex embedding~\citep{shervashidze2011weisfeiler}.
Since we test on large graphs, instead of using a learned label lookup dictionary we use a standard hash function for label shortening at each step. 
In each of the above, the outputs of the last layer are fed to a $Q$-learning network as in \S\ref{sec: Neural Network Design}.
Unlike \gtos the depth of the above neural network (NN) models are fixed across input instances. 
We also consider the following well-known (non-learning based) heuristics for each problem:
(5) {\em Greedy algorithms},
(6) {\em List heuristic},
(7) {\em Matching heuristic}. 
We refer to Appendix~\ref{sec: heuristics} for details on these heuristics. 

We attempt to compute the optimal solution via the Gurobi optimization package~\citep{gurobi}. We run the Gurobi solver with a cut-off time of 240~s, and  
% In most cases, the solver found the optimal solution for graphs of up to size 200 before this time. 
report performance in the form of approximation ratios relative to the solution found by the Gurobi solver. We do not compare against Deepwalk~\citep{perozzi2014deepwalk} or node2vec~\citep{grover2016node2vec} since these methods are designed for obtaining vertex embeddings over a single graph. 
They are inappropriate for models that need to generalize over multiple graphs. 
This is because the vertex embeddings in these approaches can be arbitrarily rotated without a consistent `alignment' across graphs. 
The number of parameters can also grow linearly with graph size. 
We refer to~\citet[Appendix D]{hamilton2017inductive} for details. 

\begin{figure*}[t]
  \centerline{
     \includegraphics[height=37mm]{figures/er_training/er_training.pdf}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: er greedy}
%     \subfigure[]{\includegraphics[height=27mm]{figures/er_training/regular}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%    \label{fig: er regular}}
%     \subfigure[]{\includegraphics[height=27mm]{figures/er_training/bipartite}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%     \label{fig: er bipartite}}
     }
     \vspace{-2mm}
    \caption{\small Minimum vertex cover in worst-case graphs for greedy (left), random regular graphs (center), and random bipartite graphs (right), using models trained on size-15 Erdos-Renyi graphs. Each point shows that average and standard deviation for 20 randomly sampled graphs of that type. The worst-case greedy graph type, however, has only one graph at each size; hence, the results show outliers for this graph type.}
    \label{fig: er_trained}
    \vspace{-15pt}
\end{figure*}


\noindent {\bf Training.}
We train \gtos, Structure2Vec, GraphSAGE and WL kernel NN all on small Erdos-Renyi (ER) graphs of size 15, and edge probability $0.15$. 
During training we truncate the \algo representation to 5 observations (i.e., $T=5$, see Fig.~\ref{fig: neural arch}). 
In each case, the model is trained for 100,000 iterations, except WL kernel NN which is trained for 200,000 iterations since it has more parameters. 
We use experience replay~\citep{mnih2013playing}, a learning rate of $10^{-3}$, Adam optimizer~\citep{kingma2014adam} and an exploration probability that is reduced from $1.0$ to a resting value of $0.05$ over 10,000 iterations. 
The amount of noise added in the evolution ($n_v(t)$ in Equation~\ref{eq: basic filter}) seemed to not matter; we have set the noise variance $\sigma^2$ to zero in all our experiments (training and testing).
As far as possible, we have tried to keep the hyperparameters in \gtos and all the neural network baselines to be the same.  
For example, all of the networks have a vertex embedding dimension of $16$, use the same neural architecture for the $Q$-network and Adam optimizer for training. 

\noindent {\bf Testing}.
% Due to the recurrent nature of \gtos, we can use the trained parameters to unroll the \algo representation to arbitrarily lengths (\S\ref{sec: Neural Network Design}).
For any $T > 0$, let $\text{\gtos}(T)$ denote the neural network (\S\ref{sec: Neural Network Design}) in which \algo is restricted to a sequence length of $T$.
To test a graph $G(V,E)$, we feed $G$ as input to the networks $\text{\gtos}(1), \text{\gtos}(2), \ldots, \text{\gtos}(T_\mathrm{max})$, and choose the `best' output as our final output.  
For each $T$, $\text{\gtos}(T)$ outputs a solution set $S_T \subseteq V$. 
The best output corresponds to that $S_T$ having the maximum objective value. 
For e.g., in the case of MVC the $S_T$ having the smallest cardinality is the best output. 
This procedure is summarized in detail in Algorithm~\ref{algo: graph2seq testing} 
in Appendix~\ref{sec: net arch appendix}.
We choose $T_\mathrm{max}=15$ in our experiments.
The time complexity of \gtos is $O(|E|T_\mathrm{max} + |V|)$.

To test generalization across graph types, we consider the following graph types: 
(1) ER graphs with edge probability $0.15$; 
(2) random regular graphs with degree $4$;  
(3) random bipartite graphs with equal sized partites and edge probability $0.75$; 
(4) worst-case examples, 
% We consider constructive examples for which the greedy heuristic has the worst approximation ratio.  
such as the worst-case graph for the greedy heuristic on MVC, which has a $O(\log n)$ approximation factor~\cite{johnson1973approximation}.
(5) Two-dimensional grid graphs, in which the sides contain equal number of vertices. 
For each type, we test on graphs with number of vertices ranging from 25--3200 in exponential increments (except WL embedding which is restricted to size 100 or 200 since it is computationally expensive).
Some of the graphs considered are dense---e.g., a 3200 node ER graph has 700,000 edges; a 3200 node random bipartite graph has 1.9 million edges.
We also test on sparse ER and bipartite graphs of sizes $10,000$ and $25000$ with an average degree of 7.5.

\subsection{Scalability and Generalization across Graph Types} \label{sec: scalability}

{\bf Scalability.}
To test scalability, we train all the NN models on small graphs of a type, and test on larger graphs of the same type. 
For each NN model, we use the {\em same} trained parameters for all of the test examples in a graph type.
We consider the MVC problem and train on: (1) size-15 ER graphs, and (2) size-20 random bipartite graphs.  
The models trained on ER graphs are then tested on ER graphs of sizes 25--3200; similarly the models trained on bipartite graphs are tested on bipartite graphs of sizes 24--3200.
We present the results in Fig.~\ref{fig: scalability}.
We have also included non-learning-based heuristics for reference.
In both ER and bipartite graphs, we observe that \gtos generalizes well to graphs of size roughly 25 through 3200, even though it was trained on size-15 graphs. 
Other NN models, however, either generalize well on only one of the two types (e.g., Structure2Vec performs well on ER graphs, but not on bipartite graphs) or do not generalize in both types. 
% \gtos~exhibits good generalization even on bipartite graphs by being consistently within 1\% of optimal at all sizes. 
\gtos~generalizes well to even larger graphs.
Fig.~\ref{fig: large table} presents results of testing on size 10,000 and 25,000 ER and random bipartite graphs.
We observe the vertex cover output by \gtos~is at least 100 nodes fewer than Structure2Vec.

{\bf Generalization across graph types.}
% \todo{mention greedy has outliers because its just one graph.}
Next we test how the models generalize to different graph types. 
We train the models on size-15 ER graphs, and test them on three graph types: (i) worst-case graphs, (ii) random regular graphs, and (iii) random bipartite graphs. 
For each graph type, we vary the graph size from 25 to 3200 as before. 
Fig.~\ref{fig: er_trained} plots results for the different baselines. 
% We make the following observations: 
% (a) 
In general, \gtos~has a performance that is within 10\% of the optimal, across the range of graph types and sizes considered.
The other NN baselines demonstrate behavior that is not consistent and have certain classes of graph types/sizes where they perform poorly.
% (b) For each graph type, there is a NN model that performs comparably to \gtos: Structure2Vec in ER and random regular graphs, GraphSAGE-pool in worst-case graphs, WL and WL-NN in random bipartite graphs. 
% This suggests that dynamically selecting the depth (recall the baseline NN models have different depths), or aggregation, depending on the input instance could result in potentially more robust graph algorithms. 

%(b) The Greedy baseline has a near-optimal performance on random bipartite graphs.
%It is slightly worse than \gtos~on random regular graphs, and does very poorly (not surprisingly) on the worst-case examples.
%(c) The GCNN baseline shows comparable performance to \gtos~and Greedy on random regular graphs.
%However it does poorly on random bipartite graphs of size 200 or less.
%On the worst-case example, the heuristic does not do well at sizes 50 or above.
%(e) The matching heuristic is consistently bad in all categories, and stays close to its approximation bound of 2. 
%(f) The list heuristic of~\citet{shimizu2016fast} has a comparable performance to \gtos~in most cases. However in random regular graphs of size $>$ 400, we observe its performance degrading more than 10\% above \gtos. 
%Thus \gtos~can not only scale within Erdos-Renyi graphs, but also across different graph types for MVC.
%In the following section, we investigate \gtos's generalization in other graph problems. 

{\bf Adversarial training.}
We also trained \gtos on a certain class of adversarial `hard' examples for minimum vertex cover, and observed further improvements in generalization.
We refer to Appendix~\ref{apx: eval} for details and results of this method. 

\subsection{Other Problems: MC and MIS} \label{sec: mc and mis}

We test and compare \gtos~on the MC and MIS problems. 
As in MVC, our results demonstrate consistently good scalability and generalization of \gtos~across graph types and sizes.
As before, we train the NN models on size-15 ER graphs ($p=0.15$) and test on different graphs. 

\noindent {\bf Max cut.}
We test on 
(1) ER graphs, and (2) two-dimensional grid graphs. 
For each graph type, we vary the number of vertices in the range $25$--$3200$, and use the same trained model for all of the tests. 
The results of our tests are presented in Fig.~\ref{fig: maxcut}.
We notice that for both graph types \gtos~is able to achieve an approximation less that $1.04$ times the (timed) integer program output.   
\begin{figure}[t]
  \centerline{
    \subfigure[]{\includegraphics[height=28mm]{figures/mc/mc.pdf}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: maxcut}}
%     \subfigure[]{\includegraphics[height=28mm]{figures/mc/maxcut_grid}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%    \label{fig: maxcut_grid}}  
    \subfigure[]{\includegraphics[height=28mm]{figures/mis/mis.pdf}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: indset}}
%     \subfigure[]{\includegraphics[height=28mm]{figures/mis/indset_greedy}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%    \label{fig: indset_greedy}}
    }
    \caption{\small (a) Max cut in Erdos-Renyi graphs (left), Grid graphs (right). (b) Maximum independent set in Erdos-Renyi graphs (left), structured bipartite graphs (right). Some approximation ratios are less than 1 due to the time cut-off of the Gurobi solver.}
    \label{fig: mcandindset}
      \vspace{-18pt}
\end{figure}
\\ \noindent {\bf Maximum independent set.}
We test on (1) ER graphs, and (2) worst-case bipartite graphs for the greedy heuristic.
The number of vertices is varied in the range 25--3200 for each graph type. 
We present our results in Fig.~\ref{fig: indset}.
In ER graphs, \gtos~shows a reasonable consistency in which it is always less than 1.10 times the (timed) integer program solution. 
%The highest approximation ratio occurs with moderate graph sizes (100 -- 400). 
% But even in this regime it is comparable to the other heuristics. 
In the bipartite graph case we see a performance within 8\% of optimal across all sizes. 
% Greedy and list heuristics do very well on Erdos-Renyi graphs, with comparable performance to \gtos~up to moderate sizes.
% However, on the bipartite graphs they have poor performance. 
% The GCNN heuristic also does moderately well on Erdos-Renyi graphs (though it is worse than both \gtos~and Greedy at all sizes). 
% As with Greedy, it progressively becomes worse (close to an approximation ratio of $2$) on the bipartite graphs. 


%(2) Structured bipartite graphs. 
%We construct an adversarial class of bipartite graphs for the Greedy heuristic.
%For a parameter $m\in 2\mathbb{N}$ we will describe a construction having $3m/2 + 2$ vertices. 
%The maximum independent set size is $m$, while Greedy chooses a set of size $m/2 + 2$ giving an approximation ratio close to 2. 
%Note that the construction below can be easily modified to generate arbitrarily high ($ > 2$) constant approximation ratios for Greedy. 
%The first partite consists of $m$ vertices $\{u_1, \ldots, u_m\}$ and the second partite consists of $m/2 + 2$ vertices $\{v_1, \ldots, v_{m/2 + 2} \}$. For $i=1,\ldots,m/2$ each $v_i$ is connected to $u_{2i-1}$ and $u_{2i}$. 
%Whereas $v_{m/2 + 1}$ and $v_{m/2 + 2}$ are connected to all of $\{u_1,\ldots, u_m \}$. \\


%We compare \algo~with the following heuristics:
%(1) Greedy, a simple $\Delta + 1$ approximation heuristic (where $\Delta$ is the maximum degree) that greedily selects vertices having the least degree as part of the independent set, and
%
%
%
%We compare \algo~with the following two heuristics: 
%(1) Greedy, a simple 2-approximation algorithm which greedily swaps vertices across the cut sets  to strictly increase the cut value, and 







%(d) The GCNN baseline trained on planted-vertex cover examples demonstrates poor approximation ratios in all graph categories.
%
%In our RL framework, we define the set of vertices chosen as actions to be our vertex cover output.
%Each time a vertex $v$ is chosen, the learning agent receives a reward of $-1$ and we set $c_v \leftarrow 1$ for all subsequent iterations.
%During each iteration we pick as action the vertex having the highest $Q$-value and has not be chosen already (i.e., for which $c_v$ is $0$).
%The algorithm terminates when there is no more edge to be covered.

% (our empirical findings stay roughly the same for $d \geq 8$. 



%To understand what aspects of the MVC algorithm are learned, we conduct empirical studies on the \algo~dynamics and present techniques for semantic interpretation. 
%The most interesting semantics are observed in the $Q(\cdot)$ function, which we recall has two terms (cf.\ Equation~\eqref{eq: Q func est}). The first term, denoted by $Q_1$,  is the same for all the vertices and includes a sum of all the $\mathbf{y}(\cdot)$ vectors. The second term, denoted by $Q_2(v)$ depends on the $\mathbf{y}(\cdot)$ vector for the vertex being considered. 
%
%We observe the values of these terms for a size-15 planted vertex cover graph, and note the following:   
%(a) the values of $Q_1$ and $Q_2(\cdot)$ are close to being integers.
%$Q_1$ has a value that is one less than the negative of the minimum vertex cover size.
%(b) For a vertex $v$, $Q_2(v)$ is binary valued from the set $\{0, 1\}$.
%$Q_2(v)$ is one, if vertex $v$ is part of an optimum vertex cover, and zero otherwise.
%Thus the neural network, in principle, computes the complete set of vertices for the optimum cover at the very first round itself. 
%A detailed list of this and other semantics is in Appendix~\ref{sec: vc geometry and sem}.

%\subsection{Testing} \label{sec: vc testing}
%
%
%
%{\bf Baseline}.  We compare our results against the following baseline algorithms: \\
%(3) Fixed-depth GCNN trained on planted vertex-cover graphs. This baseline is the same as above, but trained on the adversarial  planted-cover examples of Section~\ref{sec: VC training}. \\




%\subsection{Design Choices} \label{sec: ablation analysis}

%- why forget gate looks that sum of mu's (refer to Figs.~\ref{fig: q_val_ours_pc} and~\ref{fig: q_val_lsong_pc})

%- Complexity of ours is obviously higher compared to fixed depth; asymptotic complexity is an interesting question;

%- choice of relu (other things don't seem to work)

%- on the other hand larger is not always better due to 'structural noise'

%- choice of training set


==> arxiv 3/graph2seq.tex <==
\section{Graphs as Dynamical Systems} \label{sec: rep graphs as ts}

%\red{Change Fig. 1. Illustrate only \algo. LSTM part should go.}
%\red{Don't use 'convolutional filter' anywhere}
%\red{Include separate \algo~figure from the perspective of an individual node.}

\subsection{The \algo Representation} \label{sec: grep proof}

%\begin{figure}[t]
%    \centering
%  \includegraphics[width=.28\textwidth]{figures/dandelion}
%  \caption{Dandelion spreading forwards a message in a line over the graph, then broadcasts it using diffusion. Here both phases occur over the same graph, i.e., $H=G$.}
%  \label{fig:dandelion}
%\end{figure}

The key idea behind \algo is to represent vertices of a graph by the trajectory of an appropriately chosen dynamical system induced by the graph.
Such a representation has the advantage of progressively capturing more and more information about a vertex as the trajectory unfolds.
Consider a directed graph $G(V,E)$ whose vertices we want to represent (undirected graphs will be represented by having bi-directional edges between pairs of connected vertices).
We create a discrete-time dynamical system in which vertex $v$ has a state of ${\bf x}_v(t) \in \mathbb{R}^d$ at time $t\in\mathbb{N}$, for all $v\in V$, and $d$ is the dimension of the state space.
In \algo, we consider an evolution rule of the form
% \begin{align}
% {\bf x}_v(t+1) = g(\{ {\bf x}_u(t): u \in \Gamma(v) \}) + {\bf n} _v(t+1), 
% \label{eqn:basicevol} 
% \end{align}
%  $\forall v \in V, t \in \mathbb{N},$ where $g(\cdot)$ is a deterministic function that maps a set of vectors in $\mathbb{R}^d$ to another vector in $\mathbb{R}^d$, and ${\bf n}_v(\cdot)$ is a $d$-dimensional Gaussian circular noise with mean 0 and covariance $\sigma^2 I$. $u \in \Gamma(v)$ if there is a (directed) edge from $u$ to $v$ in the graph $G$.
% Specifically, we consider a function $g(\cdot)$ that results in the following update rule:
\begin{align}
{\bf x}_v(t+1) = \mathrm{relu}(\mathbf{W}_1 (\sum_{u\in \Gamma(v)} {\bf x}_u(t)) + \mathbf{b}_1 ) + {\bf n}_v(t+1),  \label{eq: basic filter}
\end{align}
$\forall v \in V,t\in\mathbb{N},$ where $\mathbf{W}_1\in \mathbb{R}^{d\times d}$, $\mathbf{b}_1 \in\mathbb{R}^{d\times 1}$ are trainable  parameters and relu$(x) = \max(x,0)$.
${\bf n}_v(\cdot)$ is a $d$-dimensional $(\mathbf{0}, \sigma^2 \mathbf{I})$ Gaussian noise, and $u \in \Gamma(v)$ if there is an edge from $u$ to $v$ in the graph $G$.
For any $v\in V$, starting with an initial value for ${\bf x}_v(0)$ (e.g., random or all zero) this equation % Equation~\eqref{eq: basic filter} 
defines a dynamical system, the (random) trajectory of which is the \algo~representation of $v$.
More generally, graphs could have features on vertices or edges (e.g.,  weights on vertices), which can be included in the evolution rule; these generalizations are outside the scope of this paper.
We use \algo($G$) to mean the set of all \algo vertex representations of $G$. 

% When used together with a system capable of summarizing the sequential information (e.g. LSTM), we get a representation technique that can scale to graphs of arbitrary size --- the larger the graph, the longer we can observe the trajectory for summarization.

% Though a sequential representation for nodes can be obtained via arbitrary neighborhood-induced maps, in practice we use convolutional filters of the form discussed in Section~\ref{sec: background} in order to keep the neural network differentiable.
% Therefore it becomes useful to study the dynamics of evolution under convolutional filters.
% We consider evolution under a canonical 1-local filter given by

% The transformation in Equation~\eqref{eq: basic filter} above is interesting due to its simplicity, while at the same time containing features common to many GCNN filters.\footnote{A brief discussion about these features is presented in Section~\ref{sec: ablation analysis}.}
% Moreover the architecture we use for our implementation (Section~\ref{sec: Neural Network Design}) also uses filters of this type.

% We create a dynamical system over the graph by cascading graph convolutional layers repeatedly.
% All of these layers share the same parameters allowing for an arbitrarily long cascade.
% The sequence of outputs from the layers form the \algo~representation.
% We note that many prior works have advocated for such a cascaded architecture (e.g.~\citet{dai2017learning}).
% However in these works, aside from using a fixed-depth GCNN, only the final output of the convolutional layers is considered as representing the graph.
% This is akin to considering the state of the dynamical system only at a specific time instance.
% In contrast, we view the entire sequence of convolutional layer outputs as representing the graph (in addition to allowing an arbitrarily long cascade).

%{\bf \algo~~= Seq2Graph}. 

{\bf \algo is invertible.}
Our first key result is that \algo's representation allows recovery of the adjacency matrix of the graph with arbitrarily high probability. 
Here the randomness is with respect to the noise term in \algo; see~\eqref{eq: basic filter}. 
In Appendix~\ref{sec: g2s equals s2g proof}, we prove:
\begin{thm} \label{thm: g2s equals s2g}
For any directed graph $G$ and associated (random) representation \algo($G$) with sequence length $t$, there exists an inference procedure (with time complexity polynomial in  $t$) that produces an estimate $\hat{G}_t$ such that   $\lim_{t\rightarrow\infty} \mathbb{P}[G \neq \hat{G}_t] = 0$.
\end{thm}

Note that there are many ways to represent a graph that are lossless. 
For example, we can simply output the adjacency matrix row by row.
However such representations depend on assigning {\em labels} or identifiers to vertices, which would cause downstream deep learning algorithms to memorize the label structure and not generalize to other graphs. 
\algo's key property is that it is does not depend on a labeling of the graph.
Theorem~\ref{thm: g2s equals s2g} is particularly significant (despite the representation being infinite dimensional) since it shows lossless label-independent vertex representations are possible. 
To our understanding this is the first result making such a connection.
Next, we show that the noise term in \algo's evolution rule (\eqref{eq: basic filter}) is crucial for Theorem~\ref{thm: g2s equals s2g} to hold (proof in Appendix~\ref{sec: deterministic rule proof}). 

%In this section, we show that such an additive noise term is necessary in \algo.
\begin{prop} \label{prop: deterministic rule}
Under any deterministic evolution rule of the form in~\eqref{eq: basic filter}, there exists a graph $G$ which cannot be reconstructed exactly from its \algo~representation with arbitrarily high probability.
\end{prop}
The astute reader might observe that invertible, label-independent representations of graphs can be used to solve the graph isomorphism problem~\cite{schrijver2003combinatorial}. However, Proposition~\ref{prop: deterministic rule} shows that \algo cannot solve the graph isomorphism problem, as that would require a {\em deterministic} representation.
Noise is necessary to {\em break symmetry} in the otherwise deterministic dynamical system. 
%Observe that vertices in the graph are not explicitly assigned unique identifiers.
 Observe that the time-series for a vertex in~\eqref{eq: basic filter} depends {\em only} on the time-series of its neighboring nodes, not any explicit vertex identifiers. As a result, two graphs for which all vertices have exactly the same neighbors will have exactly the same representations, even though they may be structurally different.  The proof of Proposition~\ref{prop: deterministic rule} illustrates this phenomenon for regular graphs.
 


%Since vertices lack labels, a deterministic evolution function cannot distinguish between vertices in certain symmetric graphs. The proof of Proposition~\ref{prop: deterministic rule} provides an example of this phenomenon for regular graphs that are structurally different but for which any determinstic evoluton 

%The deterministic evolution function, together with lack of identifying labels on vertices make distinguishing vertices difficult. The proof of Proposition 1 illustrates this for regular graphs. 


%The following result highlights the importance of randomization (proof in Appendix~\ref{sec: deterministic rule proof}).



% For example, consider a simple graph with two vertices $u, v$ and an edge $(u,v)$ between them. Suppose the function $f$ outputs the size of the optimal vertex cover. The optimal cover in this case is to choose either just vertex $u$, or just vertex $v$.
% However, a deterministic evolution rule would be completely symmetric at each vertex and the trajectories of both vertices %$r(u)$ and $r(v)$
% would be identical, leading to indecisiveness in choosing one of the vertices arbitrarily.

%  --- vertices are represented purely based on how they are connected to the rest of the graph.
% These two attributes together can make symmetry breaking, such as described in Section~\ref{sec: geo of encode}, difficult.
% In Section~\ref{sec: fixed length rep} we have argued that sequential representations are strictly better than fixed-length representations.
% However the capability of a sequential representation crucially depends on how the dynamics is generated.
% In particular, we note two attributes in our current \algo~design:
% (1) Nodes in the graph, besides intrinsic features they may have, are not explicitly assigned unique identifiers.
% (2) The graph convolutional filters used to create the evolution are deterministic transformation functions.

% Nevertheless in practice we see good approximation performance with our representation even on regular graphs (Section~\ref{sec: vc testing}).
% The deterministic evolution function, together with lack of identifying labels on nodes make distinguishing nodes difficult for the neural network --- vertices are represented purely based on how they are connected to the rest of the graph.

% In contrast, traditional computer science algorithms have always relied on vertex/edge identifiers for bookkeeping, even if the function to be computed does not depend on them.
% Such an architecture, if we are able to mimic on neural networks, would be ideal.
% The challenge here is to teach the neural network to use identifiers purely for bookkeeping, and not use them directly in any way for computing the intended function.

% - cite blog
%- adding noise not just to aid training
%- what about randomness in policy gradient?

\subsection{Formal Computation Model} 
\label{sec: formal model}
Although \algo~is an invertible representation of a graph, it is unclear how it compares to other GCNN representations in the literature. Below we define a formal computational model on graphs, called \model, that includes \algo~as well as a large class of GCNN representations  in the literature.
Abstracting different representations into a formal computational model allows us reason about the fundamental limits of these methods.
We show that GCNNs with a fixed number of convolutional steps cannot compute certain functions over graphs, where a sequence-based representation such as \algo~is able to do so.  For simplicity of notation, we consider undirected graphs in this section and in the rest of this paper.

%\subsubsection{\model~Model}

{\bf \model~model}.  Consider an undirected graph $G(V,E)$ on which we seek to compute a function $f: \mathcal{G} \rightarrow \mathbb{R}$, where $\mathcal{G}$ is the space of all undirected graphs.  %\footnote{We use the term function loosely -- $f$ could also be a relation or an arbitrary task.}
In the $k$-\model~model, computations proceed in two rounds: %the {\em local} step, and the {\em gather} step.
In the {\em local step}, each vertex $v$ computes a representation $r(v)$ that depends only on the subgraph of vertices that are at a distance of at most $k$ from $v$. %\footnote{For the purpose of defining our computational model, we think of the graph as being unweighted and include any node/edge weights as part of the feature space.}
Following this, in the {\em gather step}, the function $f$ is computed by applying another function $g(\cdot)$ over the collection of vertex representations $\{ r(v) : v \in V \}$.
\algo~is an instance of the $\infty$-\model~model. 
GCNNs that use localized filters with a global aggregation (e.g., \citet{kipf2016semi, dai2017learning}) also fit this model (proof in Appendix~\ref{sec: gcnn belong to model proof}).
\begin{prop} \label{ex: gcnn belong to model}
The spectral GCNN representation  in~\citet{kipf2016semi} and the spatial GCNN representation in \cite{dai2017learning}  belong to the $4$-\model~model.
\end{prop}


{\bf Fixed-length representations are insufficient}. %\label{sec: fixed length rep}
We show below that for a fixed $k>0$, no algorithm from the $k$-\model~model can compute certain 
canonical graph functions exactly (proof in Appendix\ref{sec: fixed length insuf proof}).

\begin{thm} \label{thm: fixed length insuf}
For any fixed $k>0$, there exists a function $f(\cdot)$ and an input graph instance $G$ such that no $k$-\model~algorithm can compute $f(G)$ exactly.
\end{thm}

For the graph $G$ and function $f(\cdot)$ used in the proof of Theorem~\ref{thm: fixed length insuf}, we present a sequence-based representation (from the $\infty$-\model) in Appendix~\ref{sec: seq heur trees} that is able to asymptotically compute $f(G)$. 
This example demonstrates that sequence-based representations are more powerful than fixed-length graph representations in the \model~model. Further, it illustrates how a trained neural network can produce sequential representations that can be used to compute specific functions.

 {\bf \algo and graph kernels.} 
Graph kernels~\citep{yanardag2015deep, vishwanathan2010graph, kondor2016multiscale} are another popular method of representing graphs. 
The main idea here is to define or learn a vocabulary of substructures (e.g., graphlets, paths, subtrees), and use counts of these substructures in a graph as its representation. 
The Weisfeiler-Lehman (WL) graph kernel~\citep{shervashidze2011weisfeiler, weisfeiler1968reduction} is closest to \algo. 
Starting with `labels' (e.g., vertex degree) on vertices, the WL kernel iteratively performs local label updates similar to~\eqref{eq: basic filter} but typically using discrete functions/maps. 
The final representation consists of counts of these labels (i.e., a histogram) in the graph. 
Each label corresponds to a unique subtree pattern.
However, the labels themselves are not part of any structured space, and cannot be used to compare the similarity of the subtrees they represent. 
Therefore, during testing if new unseen labels (or equivalently subtrees) are encountered the resulting representation may not generalize. 

% The final representation consists of only counts of these labels (i.e., a histogram) without the labels themselves explicitly being part of the representation.
 
% For e.g., the $k$-hop WL graph kernel~\citep{weisfeiler1968reduction} counts distinct subtree patterns of depth up to $k$ in a graph. 
% However, a graph kernel representation may not be scalable if the substructure vocabulary is limited. 
% For e.g., a test graph could have a subtree pattern that is not in the vocabulary because it was not seen during training. 

%- the local-gather algorithms discussed so far may be thought of as adaptations of the Weisfeiler-Lehman (WL) algorithm for testing graph isomorphism~\citep{weisfeiler1968reduction}.
%- Starting with labels on vertices, the WL algorithm proceeds in iterations where at each iteration labels of neighbors of a vertex are aggregated, sorted and compressed into short labels via a lookup table 



  %can potentially operate in trained neural networks.
%The heuristic can (asymptotically) compute the minimum vertex cover size on all tree graphs, including the examples $G_1$ and $G_2$ considered in Theorem~\ref{thm: fixed length insuf}.
%Though computing minimum vertex cover on trees is fairly straightforward in the traditional Turing machine model, we have explicitly designed our heuristic to fit the  neural computation model.
%Such a heuristic can

%Thus vertices having only a local knowledge of the graph around them may not be suffice for certain applications.
%On the other hand, using localized transformation functions is perhaps currently the only known neural network representation technique that can be efficiently applied on graphs of arbitrary shape and size (even if they do not work well, at large scales).
%As such our proposed heuristic \algo~represents graphs using  an unlimited sequence of local transformations.

%\subsection{Geometry of \algo~Dynamics} \label{sec: geo of encode}
%
%Understanding how the graph structure is being encoded in the dynamics of Equation~\eqref{eq: basic filter} involves answering questions such as:
%Does Equation~\eqref{eq: basic filter} have a fixed point?
%Are there values for parameters $\mathbf{W}_0$ and $\mathbf{b}_1$ that recover some basic graph properties (e.g., the adjacency matrix)?
%While a full theoretical analysis of Equation~\eqref{eq: basic filter} appears challenging  partly due to the coupling of the ${\bf x}$ variables and the nonlinearity of the ReLU,  we report the following empirical observations that at least partially help characterize the nature of the evolution.
%
%
%We consider an experiment in which $d=16$, and the entries of $\mathbf{W}_0, \mathbf{b}_1$ are drawn from an i.i.d.\ uniform over [0,1]. The state vector ${\bf x}_v$ is initialized to zero for all vertices.
%We consider graphs of size between 10--50 and of four types: random Erdos-Renyi, random tree, random regular graphs and random bipartite graph.
%In each case we perform the recursion of Equation~\eqref{eq: basic filter} at least 10 times.
%The following general observations hold with high probability with respect to both parameter values, and the graph. Perhaps surprisingly, these observations also hold true on our model with trained parameters (e.g., for finding minimum vertex covers), as we discuss in Appendix~\ref{sec: vc geometry and sem}.
%
%{\bf (1) Convergence.}
%Depending on the variance of the initializing distribution for $\mathbf{W}_0$, the state vectors either converge to zero (small variance), or blow up (large variance).
%%- $\Theta_1$ ?
%
%{\bf (2) Dimension collapse.} Roughly half the entries in the 16-dimensional state vector quickly become zeros (in about 4 or 5 iterations) and stay at zero. The indices of these zeroed-out entries are the same in state vectors across all the vertices.
%
%{\bf (3) Principal components' alignment.}
%We compute the principal component direction of the collection of vertex state vectors at each iteration, and observe that it converges.
%Figure~\ref{fig: gen_er_pca_inn_prod} shows the absolute value of the inner product between the (normalized) principal component direction at each iteration with the principal component direction at iteration 10, for the Erdos-Renyi graph shown in Figure~\ref{fig: gen_er_graph}.
%
%{\bf (4) Principal component scores and local connectivity.}
%In each iteration, we compute the principal score (projection along principal direction) of each vertex state vector. We observe that the principal score for a vertex roughly corresponds to its `local connectivity' in the graph.
%The stronger a vertex is connected, the larger is the principal score.
%Fig.~\ref{fig: gen_er_pca} shows this effect for the graph in Fig.~\ref{fig: gen_er_graph} --- vertex 9 (bright blue) is strongly connected and has the largest principal score, while vertex 7 (dark grey) has the least score.
%
%
%\begin{figure*}[t]
%  \centerline{\subfigure[]{\includegraphics[height=35mm]{figures/gen_er_graph}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%     \label{fig: gen_er_graph}}
%%     \hfil
%     \subfigure[]{\includegraphics[height=35mm]{figures/gen_er_pca}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%     \label{fig: gen_er_pca}}
%     \subfigure[]{\includegraphics[height=35mm]{figures/gen_er_pca_inn_prod}
%%       % where an .eps filename suffix will be assumed under latex,
%%       % and a .pdf suffix will be assumed for pdflatex
%    \label{fig: gen_er_pca_inn_prod}}}
%    \caption{\small (a) Erdos-Renyi graph of size 10 considered in Figures (b) and (c), (b) vertex-wise principal component scores at each iteration, and (c) projection of the principal direction at each iteration on the principal direction of iteration 10. The vertex color and the line color in Figures (a) and (b) are matched.}
%    \label{fig: pca_gen}
%\end{figure*}
%
%% - Figure~\ref{fig: pca_gen} experiment: evolution given by M $\leftarrow$ relu(Theta1 M A + bias) where Theta1 and bias are drawn uniformly randomly between -0.5 and +0.5
%% - also 7 out of 16 rows are zeroed out.



==> arxiv 3/intro.tex <==
\section{Introduction}

%Many real-world problems often involve an interacting collection of objects or entities.
%Graphs are widely used to model pairwise relationships between objects in a variety of applications (e.g., gene interactions \cite{ozgur2008identifying}, social networks \cite{ugander2011anatomy}, etc.). Designing algorithms over graphs is therefore a topic of first order interest in various fields and applications. 
%For example, in biology the network of gene interactions is represented and studied using graphs~.
%Social networks (e.g. Facebook) use the graph of user associations (e.g. friendship) to make complex recommendation and planning decisions~\citep{ugander2011anatomy}.
%In distributed data processing frameworks, jobs often have causal dependencies which are encoded as a directed acylic graph~\citep{grandl2016g}.
%Today, most graph algorithms are designed by human experts. However, in many problems, designing graph algorithms with strong performance guarantees is very challenging. Problems often involve messy optimization tasks with several constraints, or the current algorithmic understanding is simply limited (e.g., approximation gaps in CS theory literature). %Yet in other cases, human-designed heuristics may not be the best fit for a specific application.

Graph algorithms appear in a wide variety of fields and applications, from the study of gene interactions~\citep{ozgur2008identifying} to social networks~\citep{ugander2011anatomy} to computer systems~\citep{grandl2016g}. Today, most graph algorithms are designed by human experts. However, in many applications, designing graph algorithms with strong performance guarantees is very challenging. These algorithms often involve difficult combinatorial optimization problems for which finding optimal solutions is computationally intractable or current algorithmic understanding is limited (e.g., approximation gaps in CS theory literature).

In recent years, deep learning has achieved impressive results on many tasks, from object recognition to language translation to learning complex heuristics directly from data~\citep{silver2016mastering, krizhevsky2012imagenet}. It is thus natural to ask whether we can apply deep learning to automatically learn complex graph algorithms. 
To apply deep learning to such problems, graph-structured data first needs to be {\em embedded} in a high dimensional Euclidean space. 
 {\em  Graph representation} refers to the problem of embedding graphs or their vertices/edges  in Euclidean spaces. 
Recent works have proposed several graph representation  techniques, notably, a family of representations called graph convolutional neural networks (GCNN)
 that use architectures inspired by CNNs for images~\citep{bruna2013spectral, monti2016geometric, dai2017learning, niepert2016learning, defferrard2016convolutional, hamilton2017representation, bronstein2017geometric, bruna2017community}. 
 Some GCNN representations capture signals on a fixed graph while others support varying sized graphs.
 
In this paper, we consider how to learn graph algorithms in a way that generalizes to large graphs  and graphs of different topologies. We ask: {\em Can a graph neural network trained at a certain scale perform well on orders-of magnitude larger graphs (e.g., $1000 \times$ the size of training graphs) from diverse topologies?} 
% Scalability refers to the ability for a {\em single neural network model} to perform well on test graphs of different sizes (e.g., $1000 \times$ size of training graph) and topologies.
We particularly focus on learning algorithms for combinatorial optimization on graphs. 
Prior works have typically considered applications where the training and test graphs are similar in scale, shape, and attributes, and consequently have not addressed this generalization problem.
For example, \citet{dai2017learning} train models on graph of size 50-100 and test on graphs of up to size 1200 from the same family;
\citet{hamilton2017inductive} propose inductive learning methods where they train on graphs with $15k$ edges, and test on graphs with $35k$ edges (less than $3\times$ generalization in size);  \citet{ying2018graph} train and test over the same large Pinterest graph ($3$ billion nodes).  

%To learn graph algorithms that generalize to large graphs, new {\em scalable} embeddings are required. 

%Note however, when the training and test graphs are similar in shape, size, and attributes, having a
%scalable embedding is less relevant and existing GCNN or kernel methods can work well, even on large graphs. 
%For example, in \citet{ying2018graph} both training and testing are done over a large Pinterest graph.  
%We ask:  
%  we show that existing graph representations cannot scale to large graphs and have difficulty generalizing to graphs with different shapes and structural properties.  
 
 %{\em Can a graph neural network trained at a certain scale perform well on orders-of magnitude larger graphs from diverse topologies?}
 
%{\em simultaneously} (i.e., on a single trained model,~\S\ref{sec: scalability intro}) perform well on both large and small graphs, and graphs of diverse topologies.

 % 


%Scalability here means being able to {\em simultaneously} (i.e., on a single trained model,~\S\ref{sec: scalability intro}) perform well on both large and small graphs, and graphs of diverse topologies.
%Further, understanding what properties of a graph is captured by these representations is largely an open problem; thus, there is no consensus on one accepted technique.
% , either empirically or mathematically.

 
 %However, as we show in this paper, existing representations do not scale well to large graphs and have difficulty generalizing to graphs with different shapes and structural properties~\citep{bruna2017community, bronstein2017geometric}. 
%Scalability here means being able to {\em simultaneously} (i.e., on a single trained model,~\S\ref{sec: scalability intro}) perform well on both large and small graphs, and graphs of diverse topologies.
%Further, understanding what properties of a graph is captured by these representations is largely an open problem; thus, there is no consensus on one accepted technique.
% , either empirically or mathematically.


%but understanding the similarities and differences between these representations and what properties of the graph each representation captures is largely an open question, with no consensus on one accepted technique, empirically or mathematically.  Further, a key challenge is designing a representation that can scale to graphs of arbitrary shapes and sizes~\citep{bruna2017community, bronstein2017geometric}.


We propose \algo, a {\em scalable} embedding that represents vertices of a graph as a {\em time-series} (\S\ref{sec: rep graphs as ts}). Our key insight is that the fixed-sized vector representation produced by prior GCNN designs limits scalability. Instead, \algo uses the entire time-series of vectors produced by graph convolution layers as the vertex representation. This approach has two benefits: (1) it can capture subgraphs of increasing diameter around each vertex as the timeseries evolves;  (2) it allows us to vary the dimension of the vertex representation based on the input graph; for example, we can use a small number of graph convolutions during training with small graphs and perform more convolutions at test time for larger graphs.  We show both theoretically and empirically that this time-series representation significantly improves the scalability and generalization of the model. Our framework is general and can be applied to various existing GCNN architectures.

%Unlike prior works, which typically represent graphs as fixed-sized vectors, \algo provides a capability to also scale the graph representation as the input graph scales. 
%Such a framework scales to arbitrary-sized graphs and can capture structural properties that fixed-sized representations cannot capture. 
%While our framework can be thought of as a new graph neural network, our ideas are general and may also be viewed as a technique to augment existing GCNN architectures for scalability. 

% representing a graph as a timeseries, \algo scales to arbitrary-sized graphs and can capture  structural properties that fixed-sized representations cannot capture. 
 % Further, \algo can combine naturally with recurrent neural network (RNN) architectures (which process time-series data) to tackle downstream learning tasks.	


%Further, \algo makes it possible to apply recurrent neural network (RNN) architectures, which make inferences on time-series data, to learning problems on graphs.

We prove that \algo~is information-theoretically lossless, i.e., the graph can be fully recovered from the time-series representations of its vertices (\S\ref{sec: grep proof}). Our proof leverages mathematical connections between \algo and causal inference theory~\citep{granger1980testing, rahimzamani2016network, quinn2015directed}. Further, we show that \algo and many previous GCNN variants are all examples of a certain computational model over graphs that we call \model, providing for a conceptual and algorithmic unification. Using this computational model, we prove that unlike \algo, fixed-length representations fundamentally cannot compute certain functions over graphs.


%We do this by making mathematical connections between \algo~and causal inference, which is the  study of the cause-effect relationship among interacting entities by observing the dynamics of generated data~\cite{granger1980testing, rahimzamani2016network, quinn2015directed}.

%Using results developed there, we show that \algo's dynamics allows for a full recovery of the graph.

%The main advantage of \algo~is that one can harness the recent successes of recurrent neural network (RNN) architectures that make inferences on time-series data. 

To apply \algo, we combine graph convolutions with an appropriate RNN that processes the time-series representations (\S\ref{sec: Neural Network Design}). We use this neural network model, \gtos, to tackle three classical combinatorial optimization problems of varying difficulty using reinforcement learning: {\em minimum vertex cover, maximum cut} and {\em maximum independent set} (\S\ref{sec: evals}).  Our experiments show that \algo performs as well or better than the best non-learning heuristic on all three problems and exhibits significantly better scalability and generalization than previous state-of-the-art GCNN~\citep{dai2017learning, hamilton2017inductive, lei2017deriving} or graph kernel based~\citep{shervashidze2011weisfeiler} representations. Highlights of our experimental findings include: 
\begin{enumerate}[noitemsep, topsep=0pt]
\item \gtos~models trained on graphs of size 15--20 scale to graphs of size 3,200 and beyond. To conduct experiments in a reasonable time, we used graphs of size up to 3,200 in most experiments. However, stress tests show similar scalability even at 25,000 vertices.  
\item \gtos~models trained on one graph type (e.g., Erdos-Renyi) generalize to other graph types (e.g., random regular and bipartite graphs). 
\item \gtos exhibits strong scalability and generalization in each of minimum vertex cover, maximum cut and maximum independent set problems. 
\item Training over a carefully chosen adversarially set of graph examples further boosts \gtos's scalability and generalization capabilities. 
\end{enumerate}



%A key feature of our design is that the length of the \algo~representation processed by the RNN is not fixed, but can be varied according to the size and complexity of the input graph instances.  
%This provides a way to tailor the representation length to the input graph instance, increasing training and testing efficiency. 

%dynamic testing architecture provides an efficient way to process \algo's infinite sequences.  


% The adversarial choice of the training set and the {\em dynamically varying testing architecture} are the key deep learning innovations of this paper and are perhaps of broader interest. 
 
%\XXXNote{I don't we can cut the previous summary of results in the interest of space. I tried making all the important points in above. Also, I think we should discuss adversarial training as part of our experimental results. Can you take a stab at summarizing the results. I think you can write one bullet for each section of eval. Finally, it would be nice if the intro had forward references to the sections were the point being discussed appears.}

%On these combinatorial problems of varying complexity-theoretic hardness, we show that \algo~performs very well compared to state-of-the-art heuristics and shows significantly better performance and generalization than previous GCNN representations in the literature. 


% [IS THERE A SENTENCE WE CAN ADD HERE THAT SUMMARIZE HOW MUCH BETTER OUR APPROACH SCALES COMPARED TO PREVIOUS WORK. SCALABILITY IS A MAIN FOCUS SO GOOD TO HIGHLIGHT HERE]

%, where scalability is a natural issue

% {\bf Summary of Results}. \\
% %Our main results are summarized in the following. \\
% {\em(1) \algo~framework.}
% We propose a general {\em invertible} technique for representing arbitrary graphs as an infinite time-series. %, that can preserve relevant structural information regardless of the graph size.
% \algo~naturally combines with RNN architectures and reinforcement learning frameworks  for downstream graph-optimization applications resulting in new  state-of-the-art empirical performance.  \\	
% {\em (2) Fundamental limits.}
% We define a formal computational model, that encapsulates \algo~as well as various GCNN representations in the literature, and study its fundamental limits.
% We show that fixed-length representations are fundamentally limited in their capabilities and are strictly inferior to the infinite time-series representation.  \\
% {\em (3) Evaluations.}
% We demonstrate the representation capability of \algo~in conjunction with a learning architecture involving RNNs by computing the minimum vertex cover, max cut and maximum independent sets of a graph.
% These are well-known NP-hard problems with varying hardness of approximations.
% We train on a {\em single, adversarially chosen} family of graphs of size 15, and demonstrate generalization to graphs of much larger sizes (example: 800) and across diverse graph structures. The adversarial choice of the training set and the {\em dynamically varying testing architecture} are the key deep learning innovations of this paper and are perhaps of broader interest. \\
% %This is possible due to a combination of unique training strategy, and testing architecture afforded by the \algo~design. \\
% {\em (4) Semantics of representation and learning.}
% We provide a coherent semantic understanding of \algo's dynamics, both during test and training stages and  present techniques that help visualize the dynamics in the learned model.

%{\bf Related Work}.  

%\section{Graph Algorithms and Scalability} \label{sec: scalability intro}
%
%Before presenting our results we briefly discuss the nature of problems we consider and our scalability goals.
%We then present empirical evidence that naturally motivates \algo. 
%
%Our work focuses on learning combinatorial algorithms for graphs. 
%While prior work on graph neural networks is vast, our setting differs from them in a few ways.
%First, we seek to compute functions over graphs in which there is no additional data (e.g., labels, annotations, features) associated with either the nodes or the edges. 
%Examples of such functions include the diameter of the graph, chromatic number, minimum vertex cover etc. 
%Second, we seek to learn algorithms that can work well on graphs of {\em any} size and topology for such functions. 
%Traditional algorithm design in the CS community has been of this type---e.g., the Dijkstra's shortest path algorithm can compute the exact shortest path on arbitrary graphs; 
%the 2-approximation heuristic for minimum vertex cover has a guaranteed 2-approximation regardless of the size of the graph. 
%In stark contrast, state-of-the-art neural network solvers for combinatorial optimization~\citep{vinyals2015pointer, bello2016neural, dai2017learning, kool2018attention} demonstrate a graph size-dependent performance (typically considering graphs with at most a few 10s or 100s of nodes~\citep{dai2017learning, kool2018attention}), and a generalization to graph sizes at most  $10\times$ the training size. 
%
%To develop scalable graph algorithms, we first perform experiments that illustrate limitations of existing approaches. 
%We consider three recent GCN proposals~\citep{dai2017learning, li2015gated, kipf2016semi}, adapt them for computing the minimum vertex cover, and test on a wide range of graph sizes. 





==> arxiv 3/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> arxiv 3/netdesign.tex <==
\section{Section~\ref{sec: Neural Network Design} Details}
\label{sec: net arch appendix}

\begin{algorithm}[t]
   \caption{Testing procedure of \algo~on a graph instance.}
   \label{algo: graph2seq testing}
\begin{algorithmic}
   \STATE {\bfseries Input:} graph $G$, trained parameters, objective $f:G\rightarrow \mathbb{R}$ we seek to maximize, maximum sequence length $T_\mathrm{max}$
   \STATE {\bfseries Output:} solution set $S\subseteq V$
   \STATE $S_\mathrm{opt} \leftarrow \{ \}$, $v_\mathrm{opt} \leftarrow 0$ \COMMENT{initialize}
   \FOR{$T$ from $1$ {\bfseries to} $T_\mathrm{max}$}
   	\STATE $S \leftarrow $ solution returned by \algo($T$)
   		\IF{$f(S) > v_\mathrm{opt}$}
   			\STATE $S_\mathrm{opt} \leftarrow S$
			\STATE $v_\mathrm{opt} \leftarrow f(S)$
   		\ENDIF
   \ENDFOR
   \STATE {\bf return} $S_\mathrm{opt}$
\end{algorithmic}
\end{algorithm}


%\begin{algorithm}[t]
%\DontPrintSemicolon
%\KwIn{graph $G$, trained parameters, objective $f:G\rightarrow \mathbb{R}$ we seek to maximize, maximum sequence length $T_\mathrm{max}$}
%\KwOut{solution set $S\subseteq V$}
%$S_\mathrm{opt} \leftarrow \{ \}$, $v_\mathrm{opt} \leftarrow 0$ \tcp*{initialize} 
%\For{$T$ from $1$ to $T_\mathrm{max}$} {
%$S \leftarrow $ solution returned by \algo($T$) \; 
%	\If{$f(S) > v_\mathrm{opt}$} {
%		$S_\mathrm{opt} \leftarrow S$ \;
%		$v_\mathrm{opt} \leftarrow f(S)$ \;
%	}	
%}
%\Return $S_\mathrm{opt}$
%\caption{Testing procedure of \algo~on a graph instance.}
%\label{algo: graph2seq testing}
%\end{algorithm}

\subsection{Reinforcement Learning Formulation} \label{sec: learning algorithm}
Let $G(V,E)$ be an input graph instance for the optimization problems mentioned above. 
Note that the solution to each of these problems can be represented by a set $S \subseteq V$. 
In the case of the minimum vertex cover (MVC) and maximum independent set (MIS), the set denotes the desired optimal cover and independent set respectively; 
for max cut (MC) we let $(S, S^c)$ denote the optimal cut. 
For the following let  $f:2^V \rightarrow \mathbb{R}$ be the objective function of the problem (i.e., MVC, MC or MIS) that we want to maximize, and let $\mathcal{F} \subseteq 2^V$ be the set of feasible solutions. 

{\bf Dynamic programming formulation.} Now, consider a dynamic programming heuristic in which the subproblems are defined by the pair $(G, S)$, where $G$ is the graph and $S\subseteq V$ is a subset of vertices that have already been included in the solution.  
For a vertex $a\in V \backslash S$ let $ Q(G,S, a) = \max_{S' \supseteq S\cup\{a\}, S' \in \mathcal{F}}f(S') - f(S\cup \{a\}) $ denote the marginal utility gained by selecting vertex $a$. 
Such a $Q$-{\em function} satisfies the Bellman equations given by
\begin{align}
Q(G,S,a) = &f(S\cup\{a\}) - f(S) \notag \\
&+ \max_{a' \in V \backslash S\cup\{a\} }Q(G, S\cup\{a\}, a'). \label{eq: Bellman equations}
\end{align}
It is easily seen that computing the $Q$-functions solves the optimization problem, as $\max_{S \in \mathcal{F}} f(S) = \max_{a\in V} Q(G, \{\}, a)$.   
However exactly computing $Q$-functions may be computationally expensive. 
One approach towards approximately computing $Q(G,S,a)$ is to fit it to a (polynomial time computable) parametrized function, in a way that an appropriately defined error metric is minimized. 
This approach is called $Q$-{\em learning} in the reinforcement learning (RL) paradigm, and is described below. 

{\bf State, action and reward.} We consider a reinforcement learning policy in which the solution set $S\subseteq V$ is generated one vertex at a time. 
The algorithm proceeds in rounds, where at round $t$ the RL agent is presented with the graph $G$ and the set of vertices $S_t$ chosen so far. 
Based on this {\em state} information, the RL agent outputs an {\em action} $A_t \in  V \backslash S_t$. 
The set of selected vertices is updated as $S_{t+1} = S_t \cup \{A_t\}$. 
Initially $S_0 = \{ \}$. 
Every time the RL agent performs an action $A_t$ it also incurs a {\em reward} $R_t = f(S_t\cup \{A_t\}) - f(S_t)$.
Note that the $Q$-function $Q(G, S_t, a)$ is well-defined only if $S_t$ and $a$ are such that there exists an $S' \supseteq S_t \cup \{a\}$ and $S' \in \mathcal{F}$. 
To enforce this let $\mathcal{F}_t = \{ a \in V \backslash S_t: \exists~ S' \text{ s.t. } S' \supseteq S_t \cup \{a\} \text{ and } S' \in \mathcal{F} \} $ denote the set of  feasible actions at time $t$.
Each round, the learning agent chooses an action $A_t \in \mathcal{F}_t$. 
The algorithm terminates when $\mathcal{F}_t = \{ \}$.  

{\bf Policy.} 
The  goal of the RL agent is to learn a {\em policy} for selecting actions at each time, such that the cumulative reward incurred $\sum_{t\geq 0} R_t$ is maximized. 
% Ideally, we would like a policy that universally maximizes the cumulative reward for every instance of the graph from a set or distribution of interest -- however it may not be possible.  
A measure of the generalization capability of the policy is how well it is able to maximize cumulative reward for different graph instances from a collection (or from a  distribution) of interest. 
 
{\bf $Q$-learning.}
Let $\tilde{Q}(G, S, a; \Theta)$ denote the approximation of $Q(G,S,a)$ obtained using a parametrized function with parameters $\Theta$. 
Further let $\left( (G_i, S_i, a_i) \right)_{i=1}^N$ denote a sequence of (state, action) tuples available as training examples. 
We define empirical loss as 
\begin{align}
\hat{L} = &\sum_{i=1}^N\left( \tilde{Q}(G_i,S_i,a_i; \Theta) - f(S_i\cup\{a_i\}) + f(S_i) \right. \notag \\
&\left. - \max_{a' \in V \backslash S_i\cup\{a_i\} } \tilde{Q}(G_i, S_i\cup\{a_i\}, a'; \Theta) \right)^2, \label{eq: emp loss}
\end{align}
and minimize using stochastic gradient descent. 
The solution of the Bellman equations~\eqref{eq: Bellman equations} is a stationary point for this optimization. 

{\bf Remark.} 
Heuristics such as ours, which select vertices one at a time in an irreversible fashion are studied as `priority greedy' algorithms in computer science literature~\citep{borodin2003incremental, angelopoulos2003randomized}.
The fundamental limits (worst-case) of priority greedy algorithms for minimum vertex cover and maximum independent set has been discussed in~\citet{borodin2010priority}. 

\subsection{Seq2Vec Update Equations}

{\bf Seq2Vec.}
The sequence $\left( \{\mathbf{x}_v(t): v \in V\} \right)^T_{t=1}$ is processed by a  gated  recurrent network that sequentially reads $\mathbf{x}_v(\cdot)$ vectors at each time index for all $v\in V$.
Standard GRU~\citep{chung2014empirical}.
For time-step $t\in\{1,\ldots,T\}$, let $\mathbf{y}_v(t) \in \mathbb{R}^d$ be the $d$-dimensional cell state, $\mathbf{i}_v(t)\in\mathbb{R}^d$ be the cell input and $\mathbf{f}_v(t) \in (0,1)^d$  be the forgetting gate, for each vertex $v\in V$.
Each time-step a fresh input $\mathbf{i}_v(t)$ is computed based on the current states $\mathbf{x}_u(t)$ of $v$'s neighbors in $G$.
The cell state is updated as a convex combination of the freshly computed inputs $\mathbf{i}_v(t)$ and the previous cell state $\mathbf{y}_v(t-1)$, where the weighting is done according to a forgetting value $\mathbf{f}_v(t)$ that is also computed based on the current vertex states.
The update equations for the input vector, forgetting value and cell state are chosen as follows:
\begin{align}
\mathbf{i}_v(t+1) &= \mathrm{relu} ( \mathbf{W}_4 \sum_{u\in\Gamma(v)} \mathbf{x}_v(t) + \mathbf{w}_5 c_v(t) + \mathbf{b}_6 ) \notag \\
\mathbf{f}_v(t+1) &= \mathrm{sigmoid} ( \mathbf{W}_7 \sum_{u\in V} \mathbf{x}_u(t) + \mathbf{b}_8 ) \notag \\
\mathbf{y}_v(t+1) &= \mathbf{f}_v(t+1) \odot \mathbf{i}_v(t+1) + (\mathbf{1}-\mathbf{f}_v(t+1)) \odot \mathbf{y}_v(t),
\end{align}
where $\mathbf{W}_4, \mathbf{W}_7 \in \mathbb{R}^{d\times d}$ and $\mathbf{w}_5, \mathbf{b}_6, \mathbf{b}_8 \in \mathbb{R}^d$ are trainable parameters,  $t=0,1,\ldots,T-1$, and $\mathbf{1}$ denotes the $d$-dimensional all-ones vector, and $\odot$ is element-wise multiplication. $\mathbf{y}_v(0)$ is initialized to all-zeros for every $v\in V$.
The cell state at the final time-step $\mathbf{y}_v(T), v\in V$ is the desired vector summary of the \algo~sequence.





==> arxiv 3/related.tex <==
\section{Related Work}

{\bf Neural networks on graphs.}
Early works to apply neural-network-based learning to graphs are~\citet{gori2005new, scarselli2009graph}, which consider an information diffusion mechanism.
% where nodes update their states based on the states of their neighbors until an equilibrium is reached.
The notion of convolutional networks for graphs as a generalization of classical convolutional networks for images was introduced by \citet{bruna2013spectral}.
A key contribution of this work is the definition of graph convolution in the {\em spectral domain} using graph Fourier transform theory. Subsequent works have developed local spectral convolution techniques that are easier to compute~\citep{defferrard2016convolutional, kipf2016semi}.
Spectral approaches do not generalize readily to different graphs due to their reliance on the particular Fourier basis on which they were trained.
To address this limitation, recent works have considered {\em spatial convolution} methods~\citep{dai2017learning, monti2016geometric, niepert2016learning, such2017robust, duvenaud2015convolutional, atwood2016diffusion}.
\cite{li2015gated, johnson2016learning} propose a variant that uses gated recurrent units to perform the state updates, which has some similarity to our representation dynamics; however, the sequence length is fixed between training and testing.
\citet{velivckovic2017graph, hamilton2017inductive} use additional aggregation methods such as vertex attention or pooling mechanisms to summarize neighborhood states. 
In Appendix~\ref{sec: background} we show that local spectral GCNNs and spatial GCNNs are mathematically equivalent, providing a unifying view of the variety of GCNN representations in the literature.

Another line of work~\citep{jain2016structural, marcheggiani2017encoding, tai2015improved} combines graph neural networks with RNN modules.
They are not related to our approach, since in these cases the sequence (e.g., time-series of object relationship graphs from a video) is already given as part of the input. 
In contrast our approach generates a sequence as the desired embedding from a single input graph. 
\citet{perozzi2014deepwalk, grover2016node2vec} use random walks to learn vertex representations in an unsupervised or semi-supervised fashion.
However they consider prediction or classification tasks over a fixed graph. 

% \citet{johnson2016learning}, 

\smallskip
\noindent
{\bf Combinatorial optimization.}
Using neural networks for combinatorial optimization problems dates back to the work of~\citet{hopfield1985neural} and has received considerable attention in the deep learning community in recent years. \citet{vinyals2015pointer, bello2016neural, kool2018attention} consider the traveling salesman problem using reinforcement learning. These papers consider two-dimensional coordinates for vertices (e.g. cities on a map), without any explicit graph structure.
\citet{graves2016hybrid} propose a more general approach: a differential neural computer that is able to perform tasks like finding the shortest path in a graph.
The work of \citet{dai2017learning} is closest to ours. It applies a spatial GCNN representation in a reinforcement learning framework to solve combinatorial optimization problems such as minimum vertex cover. 
% Our empirical results compare \algo to this recent baseline and demonstrate that it scales and generalize significantly better, both in graph size and across different types of graphs. Further, we prove that unlike GCNN representations, \algo is reversible.  





==> arxiv 3/trained_semantics.tex <==
\section{Evaluation Details} \label{apx: eval}

\subsection{Heuristics compared}
\label{sec: heuristics}
We compare \gtos~against: 

(1) {\em Structure2Vec}~\citep{dai2017learning}, a spatial GCNN with depth of 5. \\
(2) {\em GraphSAGE}~\citep{hamilton2017inductive} using (a) GCN, (b) mean and (c) pool aggregators, with the depth restricted to 2 in each case. \\ 
(3) {\em WL kernel NN}~\citep{lei2017deriving}, a neural architecture that embeds the WL graph kernel, with a depth of 3 and width of 4 (see~\citet{lei2017deriving} for details). \\
% Unlike \gtos the depth of the above neural network (NN) models are fixed across input instances. 
% We also consider the following well-known (non-learning based) heuristics for each problem:
(4) {\em WL kernel embedding}, in which the feature map corresponding to WL subtree kernel of the subgraph in a 5-hop neighborhood around each vertex is used as its vertex embedding~\citep{shervashidze2011weisfeiler}.
Since we test on large graphs, instead of using a learned label lookup dictionary we use a standard SHA hash function for label shortening at each step. 
In each of the above models, the outputs of the last layer are fed to a $Q$-learning network, and trained the same way as \gtos. \\
(5) {\em Greedy algorithms.}
We consider greedy heuristics~\citep{williamson2011design} for each of MVC, MC and MIS. \\
(6) {\em List heuristic.} A fast list-based algorithm proposed recently in~\citet{shimizu2016fast} for MVC and MIS. \\
(7) {\em Matching heuristic.} A $2$-approximation algorithm for MVC~\citep{williamson2011design}.

%We attempt to compute the optimal solution via the Gurobi optimization package~\citep{gurobi}. We run the Gurobi solver with a cut-off time of 240~s, and  
%% In most cases, the solver found the optimal solution for graphs of up to size 200 before this time. 
%report performance in the form of approximation ratios relative to the solution found by the Gurobi solver. We do not compare against Deepwalk~\citep{perozzi2014deepwalk} or node2vec~\citep{grover2016node2vec} since these methods are designed for obtaining vertex embeddings over a single graph. 
%They are inappropriate for models that need to generalize over multiple graphs. 
%This is because the vertex embeddings in these approaches can be arbitrarily rotated without a consistent `alignment' across graphs. 
%The number of parameters can also grow linearly with graph size. 
%We refer to~\citet[Appendix D]{hamilton2017inductive} for details. 


\subsection{Adversarial Training} \label{sec: adv training} 
\begin{figure*}[t]
  \centerline{
     \subfigure[]{\includegraphics[height=25mm]{figures/adv_training/erdos}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
    \label{fig: adv erdos}}  
     \subfigure[]{\includegraphics[height=25mm]{figures/adv_training/regular}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
    \label{fig: adv regular}}
     \subfigure[]{\includegraphics[height=25mm]{figures/adv_training/bipartite}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: adv bipartite}}
     \subfigure[]{\includegraphics[height=25mm]{figures/adv_training/greedy}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: adv greedy}}}
    \caption{\small Minimum vertex cover in (a) random Erdos-Renyi graphs, (b) random regular graphs, (c) random bipartite graphs, (d) greedy example, under Erdos-Renyi graph and adversarial graph training strategies.}
    \label{fig: adv training}
\end{figure*}

So far we have seen the generalization capabilities of a \gtos~model trained on small Erdos-Renyi graphs.
In this section we ask the question: is even better generalization possible by training on a different graph family? 
The answer is in the affirmative. 
We show that by training on {\em planted vertex-cover} graph examples---a class of `hard' instances for MVC---we can realize further generalizations. 
A planted-cover example is a graph, in which a small graph is embedded (`planted') within a larger graph such that the vertices of the planted graph constitute the optimal minimum vertex cover.
% For our training, we first generate a random Erdos-Renyi graph $G_i$ of size $5$ and edge probability $p=0.15$. 
% Next, we generate a second graph $G_o$ of size $10$ in which all the vertices are disjoint.
% The overall graph is formed by connecting each vertex of $G_o$ to each vertex of $G_i$.
% Note that the vertices of $G_i$ form the optimum vertex cover in these examples.
Figure~\ref{fig: adv training} shows the result of testing \gtos~models trained under both Erdos-Renyi and planted vertex cover graphs. 
While both models show good scalability in Erdos-Renyi and regular graphs, on bipartite graphs and worst-case graphs the model trained on planted-cover graphs shows even stronger consistency by staying 1\% within optimal. 


\subsection{Geometry of Encoding and Semantics of \algo} \label{sec: vc geometry and sem}

\begin{figure*}[th]
  \centerline{\subfigure[]{\includegraphics[height=35mm]{figures/er_graph}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: er_graph}}
%     \hfil
     \subfigure[]{\includegraphics[height=40mm]{figures/er_pca}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: er_pca}}
%     \hfil
     \subfigure[]{\includegraphics[height=40mm]{figures/er_pca_inn_prod}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
    \label{fig: er_pca_inn_prod}}}
    \caption{(a) Erdos-Renyi graph of size 10 considered in Figures (b) and (c), (b) vertex-wise principal component scores at each layer, and (c) projection of the principal direction at each iteration on the principal direction of iteration 10. These experiments are performed on our trained model.}
    \label{fig: pca_trained}
\end{figure*}

Towards an understanding of what aspect of solving the MVC is learnt by \algo, we conduct empirical studies on the dynamics of the state vectors as well as  present techniques and semantic interpretations of \algo. 
%This is done in the same spirit as in Section~\ref{sec: geo of encode}. % we have made empirical observations on some general properties of the node state vectors, under random initialization of parameters.
%In this section, we repeat a similar exercise on our trained model.
%We observe that, surprisingly, all of the properties continue to hold even in the trained model.
%In addition, we also~that may help in explaining not only our heuristic, but also other GCNN heuristics.

In the first set of experiments, we investigate the vertex state vector sequence.
We consider graphs of size up to 50 and of types discussed in Section~\ref{sec: evals}.
For each fixed graph, we observe the vertex state $\mathbf{x}(\cdot)$ (Equation~\ref{eq: basic filter}) evolution to a depth of 10 layers.

{\bf (1) Dimension collapse.}
As in the random parameter case, we observe that on an average more than 8 of the 16 dimensions of the vertex state become zeroed out after 4 or 5 layers.

{\bf (2) Principal components' alignment.}
The principal component direction of the vertex state vectors at each layer converges.
Fig.~\ref{fig: er_pca_inn_prod} shows this effect for the graph shown in Fig.~\ref{fig: er_graph}.
We plot the absolute value of the inner product between the principal component direction at each layer and the principal component direction at layer 10.

{\bf (3) Principal component scores and local connectivity.}
The component of the vertex state vectors along the principal direction roughly correlate to how well the vertex is connected to the rest of the graph.
We demonstrate this again for the graph shown in Fig.~\ref{fig: er_graph}, in Fig~\ref{fig: er_pca}.
% One significant difference here, from the random parameters case, is that the value of the principal score in the trained model do not rise as sharply as the random case (Fig.~\ref{fig: gen_er_pca}) with increasing number of layers.

%- Fig.~\ref{fig: pca_trained} experiment: fixed erdos-renyi graph of size 10 (shown in picture)
%- we run lstmv2.py on it and look at the mu matrix values in the first iteration at each layer. this is stored in 'plots and results' folder
%- we can use that file to tell the number of zeroed out rows in mu
%- pics 2 and 3 look at the PCA of the mu matrices; 2 looks at (absolute value of ) projection of mu vectors at each layer into the principal component of 10th mu matrix. vertex 5 and 8 have overlapping plot lines;
%- one observation is on the trained model, the value do not rise as sharply as on random parameters (where the rise is exponential)
%- pic 3 looks at principal component direction of mu matrix at each layer and projects it on the principal direction of the 10th mu matrix to show that the principal directions are converging
%- all of this on our trained lstm model


{\bf (4) Optimal depth}.
 We study the effect of depth on approximation quality on the  four graph types being tested (with size 50); we plot the vertex cover quality as returned by \algo as we vary the number of layers up to 25.
Fig.~\ref{fig: layerwise} plots the results of this experiment, where there is no convergence behavior but nevertheless  apparent that different graphs work optimally at different layer values.
While the optimal layer value is 4 or 5 for  random bipartite and random regular graphs,  the worst case greedy example requires 15 rounds.
This experiment underscores the importance of having a {\em flexible} number of layers is better than a fixed number; this is only enabled by the time-series nature of \algo~and is inherently missed by the fixed-depth GCNN representations in the literature.

%- what layer does optimal occur? for worst-case greedy and for erdos-renyi
%- different layers, we pick the minimum
%- Fig.~\ref{fig: layerwise} experiment: we fix one size 50 graph of types erdos-renyi, random regular (degree 4), random bipartite (p=0.75) and greedy worst case each.
%- we run lstm.py on each of those 4 graphs with varying depth and look at the approximation ratio (relative to gurobi) and plot the ratios.
%- run qtestlayerwise.py with maxnumlayers=25



{\bf (5) $Q$-function semantics.}
Recall that the $Q$-function of~\eqref{eq: Q func est} comprises of two terms.
The first term, denoted by $Q_1$,  is the same for all the vertices and includes a sum of all the $\mathbf{y}(\cdot)$ vectors. The second term, denoted by $Q_2(v)$ depends on the $\mathbf{y}(\cdot)$ vector for the vertex being considered. In this experiment we plot these two values at the very first layer of the learning algorithm (on a planted vertex cover graph of size 15, same type as in the training set) and make the following observations: (a) the values of $Q_1$ and $Q_2(\cdot)$ are close to being integers.
$Q_1$ has a value that is one less than the negative of the minimum vertex cover size.
(b) For a vertex $v$, $Q_2(v)$ is binary valued from the set $\{0, 1\}$.
$Q_2(v)$ is one, if vertex $v$ is part of an optimum vertex cover, and zero otherwise.
Thus the neural network, in principle, computes the complete set of vertices in the optimum cover at the very first round itself.


\begin{figure*}[t]
  \centerline{\subfigure[]{\includegraphics[height=46mm]{figures/layerwise}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: layerwise}}
%     \hfil
     \subfigure[]{\includegraphics[height=40mm]{figures/q_val_ours_pc}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
     \label{fig: q_val_ours_pc}}
%     \hfil
     \subfigure[]{\includegraphics[height=40mm]{figures/q_val_lsong_pc}
%       % where an .eps filename suffix will be assumed under latex,
%       % and a .pdf suffix will be assumed for pdflatex
    \label{fig: q_val_lsong_pc}}}
    \caption{(a) Approximation ratio of \algo~with varying number of layers, (b) $\mathbf{y}(\cdot)$ vectors of \algo~in the intermediate layers seen using the $Q$-function, (c) $\mathbf{x}(\cdot)$ vectors of the fixed-depth model seen using the $Q$-function. Figure (b) and (c) are on planted vertex cover graph with optimum cover of vertices $\{0,1,2,3,4\}$. }
    \label{fig: layerwise q_val}
\end{figure*}


{\bf (6) Visualizing the learning dynamics}.  The above observations suggests to `visualize' how our learning algorithm proceeds in each layer of the evolution using the lens of the value of
  $Q_2(\cdot)$. % is computed using the $\pi(\cdot)$ vector of vertices in the {\em last step} of the sequence.
%While the intermediate $\pi(\cdot)$ vector values in their raw form can be hard to interpret, we can use the second term of the $Q$-function as a `lens' through which we can meaningfully view the vectors.
In this  experiment, we consider size-15 planted vertex cover graphs on (i) \algo, and (ii) the fixed-depth GCNN  trained on planted vertex cover graphs.
%In both cases we use the corresponding $Q$-function networks to visualize the intermediate layer values.
Fig.~\ref{fig: q_val_ours_pc} and~\ref{fig: q_val_lsong_pc} show the results of this experiment.
The planted vertex cover graph considered for these figures has an optimal vertex cover comprising vertices $\{0,1,2,3,4\}$.
We center (subtract mean) the $Q_2(\cdot)$ values at each layer, and threshold them to create the visualization.
A dark green color signifies the vertex has a high $Q_2(\cdot)$ value, while the yellow means a low $Q_2(\cdot)$ value.
We can see that in \algo~the heuristic is able to compute the optimal cover, and moreover this answer does not change with more rounds.
 The fixed depth GCNN has a non-convergent answer which oscillates between  a complementary set of vertices. Take away message:  having an upper LSTM layer in the learning network is critical to identify when an optimal solution is reached in the evolution, and ``latch on" to it.

%- empirical results stored in 'plots and results' folder where we use the Q function lens to see the output pi matrices;
%- this is done on a planted clique example of size (5, 10) with the inner graph having edges (0,2), (2,3) (3,4)
%- we observe first part of Q function is close to -6 (optimal vc is 5), and the second part is either +1 or 0 (since rewards are negative, everything is negative)
%- in Figs.~\ref{fig: q_val_ours_pc} and~\ref{fig: q_val_lsong_pc} we look at the second part of the Q function for our model and Le Song model trained on size 15 planted cover;
%- we center (subtract mean) the matrices and do a colormap with threshold at +-0.25 (green is higher, yellow is smaller)
%- we observe oscillations in Le Song, while ours is stable due to the LSTM constructed on top of Le Song. Vertices 0--4 are optimal.

